Mutual-Coupling-Aware Movable and Fluid Antennas on Holographic Surfaces: A Wavenumber-Domain Circuit-Field Unification

Movable and fluid antenna systems turn antenna position into a design variable. At sub-wavelength spacings, however, their behavior is governed by mutual coupling, modeled today by two disjoint traditions: circuit-theoretic impedance matrices with element-level constants, and field-theoretic kernels with norm-type power constraints. This paper unifies the two. Starting from the impedance kernel of a holographic surface, a Poynting-anchored balance identifies its resistive part with ohmic plus radiated power and its reactive part with stored-energy imbalance, and a circuit-field equivalence shows that the multiport impedance matrix is the kernel sampled at the port separations, in a single closed spherical-Hankel form. In the wavenumber domain the resistive kernel asymptotically diagonalizes in the aperture size: visible modes radiate at closed-form prices, evanescent modes only dissipate, and a flexible port becomes a constant-modulus codeword whose coupling is the pullback of the spectral weight. Coupling-aware multi-user sum-rate maximization over precoders and port positions is then formulated under physical power and voltage constraints and solved by weighted-MMSE and projected-gradient steps with closed-form gradients. A modal relaxation upper-bounds every port configuration and seeds the search by FFT-based codeword projection. A half-wavelength corollary and a superdirectivity margin quantify when coupling hurts, and when it helps.

==> acronyms.tex <==
\acrodef{A2G}{Air-to-Ground}
\acrodef{AoV}{Angles of View}

\acrodef{BS}{Base Station}
\acrodef{BCD}{Block Coordinate Descendent}

\acrodef{CBR}{Constant BitRate}
\acrodef{CP}{Check-Point}

\acrodef{FoV}{Field of View}
\acrodef{FoVs}{Fields of View}

\acrodef{FR1}{Frequency Range 1}

\acrodef{GA}{Genetic Algorithm}

\acrodef{KPI}{Key Performance Index}
\acrodef{KPIs}{Key Performance Indices}

\acrodef{IoD}{Internet of Drones}
\acrodef{IoT}{Internet of Things}
\acrodef{ISAAC}{Iterative Stochastic ApproAch to constrained drones' Communications}
\acrodef{ITS}{Intelligent Transportation System}

\acrodef{LIDAR}{LIght Detection And Ranging}
\acrodef{LoS}{Line of Sight}

\acrodef{MEC}{Mobile Edge Computing}
\acrodef{MIMO}{Multiple-Input-Multiple-Output}
\acrodef{MINLP}{Mixed-Integer Non-Linear Programming}
\acrodef{MINLFP}{Mixed-Integer Non-Linear Fractional Programming}

\acrodef{NLFP}{Non-Linear Fractional Programming}
\acrodef{NOMA}{Non-Orthogonal Multiple Access}
\acrodef{NR-U}{5G NR in Unlicensed spectrum}
\acrodef{NLoS}{Non Line of Sight}

\acrodef{OoS}{Out-of-Service}

\acrodef{QoE}{Quality of Experience}

\acrodef{RGB}{Red Green and Blue}

\acrodef{SCA}{Successive Convex Approximation}
\acrodef{SoC}{System-on-chip}
\acrodef{SNR}{Signal-to-Noise Ratio}

\acrodef{UAV}{Unmanned Aerial Vehicle}
\acrodef{UDP}{User Datagram Protocol}

\acrodef{VLC}{Visible Light Communications}

\acrodef{WSN}{Wireless Sensor Network}
\acrodef{IRS}{Intelligent Reflective Surface}
\acrodef{RIS}{Reconfigurable Intelligent Surface}
\acrodef{PRU}{Passive Reflective Unit}
\acrodef{GU}{Ground User}
\acrodef{OFDMA}{Orthogonal Frequency Multiple Access}
\acrodef{AtG}{Air-to-Ground}
\acrodef{AoA}{Angles of Arrival}
\acrodef{AoD}{Angles of Departure}
\acrodef{RV}{Random Variable}
\acrodef{CDF}{Cumulative Distribution Function}
\acrodef{PDF}{Probability Density Function}
\acrodef{CSI}{Channel State Information}
\acrodef{DRL}{Deep Reinforcement Learning}
\acrodef{PPO}{Proximal Policy Optimization}
\acrodef{MDP}{Markov Decision Process}
\acrodef{FBS}{Flying Base Station}
\acrodef{WPT}{Wireless Power Transfer}
\acrodef{TDMA}{Time Division Multiple Access}
\acrodef{AO}{Alternating Optimization}
\acrodef{MMSE}{Minimum Mean Squared Error}
\acrodef{SINR}{Signal-to-Interference-plus-Noise Ratio}
\acrodef{MRC}{Maximum Ratio Combining}
\acrodef{LS}{Least Squares}
\acrodef{MSE}{Mean Squared Error}
\acrodef{DFT}{Discrete Fourier Transform}
\acrodef{RMSE}{Root Mean Squared Error}

\acrodef{HMIMO}{Holographic MIMO}
\acrodef{DoF}{Degrees of Freedom}
